Smells in System User Interactive Tests

Test smells are known as bad development practices that reflect poor design and implementation choices in software tests. Over the last decade, test smells were heavily studied to measure their prevalence and impacts on test maintainability. However, these studies focused mainly on the unit level and to this day, the work on system tests that interact with the System Under Test through a Graphical User Interface remains limited. To fill the gap, we conduct an exploratory analysis of test smells occurring in System User Interactive Tests (SUIT). First, based on a multi-vocal literature review, we propose a catalog of 35 SUIT-specific smells. Then, we conduct an empirical analysis to assess the prevalence and refactoring of these smells in 48 industrial test suites and 12 open-source projects. We show that the same type of smells tends to appear in industrial and open-source projects, but the symptoms are not addressed in the same way. Smells such as Obscure Test, Sneaky Checking, and Over Checking show symptoms in more than 70% of the tests. Yet refactoring actions are much less frequent with less than 50% of the affected tests ever undergoing refactoring. Interestingly, while refactoring actions are rare, some smells, such as Narcissistic, disappear through the removal of old symptomatic tests and the introduction of new tests not presenting such symptoms.

==> rq.tex <==
\section{Research questions}


We begin our investigation by looking at how well SUIT smells are covered by both the grey literature and the academic literature. The goal behind this first questions is to investigate whether or not there exist a gap between the knowledge present in the research community and among practitioners. Thus, we formulate our first research question as:

\begin{description} 
\item[\textbf{RQ1}:]
\emph{What are the SUIT smells studied in academic and grey literature?} 
\end{description} 

Once we have established a catalog of SUIT smells, we continue our endeavor by assessing to which extent the symptoms of each smells are present in SUITs. To that end, we compute the number of occurrences of the symptoms for each smell in every SUIT. In other words, for each smell we associate a metric and observe how that metric is distributed over the different tests. Therefore, we ask the following question:

\begin{description} 
\item[\textbf{RQ2}:]
\emph{How widespread are SUIT smell symptoms in SUITs?} 
\end{description} 

Finally, we focus on the refactoring actions performed by the maintainer of the test suites to remove the smell symptoms. However, because those symptoms can be removed by actions not related to the symptom removal itself but merely being the by-product of another action, we focus our analysis on fine grain changes, specifically targeting the removal of the symptom itself. Hence, we formulate our third research question as follow:

\begin{description} 
\item[\textbf{RQ3}:]
\emph{How often do we observe refactoring actions removing SUIT smell symptoms?} 
\end{description} 
